A scalable generative model for dynamical system reconstruction from neuroimaging data

Data-driven inference of the generative dynamics underlying a set of observed time series is of growing interest in machine learning and the natural sciences. In neuroscience, such methods promise to alleviate the need to handcraft models based on biophysical principles and allow to automatize the inference of inter-individual differences in brain dynamics. Recent breakthroughs in training techniques for state space models (SSMs) specifically geared toward dynamical systems (DS) reconstruction (DSR) enable to recover the underlying system including its geometrical (attractor) and long-term statistical invariants from even short time series. These techniques are based on control-theoretic ideas, like modern variants of teacher forcing (TF), to ensure stable loss gradient propagation while training. However, as it currently stands, these techniques are not directly applicable to data modalities where current observations depend on an entire history of previous states due to a signal's filtering properties, as common in neuroscience (and physiology more generally). Prominent examples are the blood oxygenation level dependent (BOLD) signal in functional magnetic resonance imaging (fMRI) or Ca$^{2+}$ imaging data. Such types of signals render the SSM's decoder model non-invertible, a requirement for previous TF-based methods. Here, exploiting the recent success of control techniques for training SSMs, we propose a novel algorithm that solves this problem and scales exceptionally well with model dimensionality and filter length. We demonstrate its efficiency in reconstructing dynamical systems, including their state space geometry and long-term temporal properties, from just short BOLD time series.

==> short_long_aln_comparison.tex <==
\begin{table}
\centering
\caption{Results of the PLRNN with BOLD observation model on the ALN dataset. 1000 models                                                                                        are trained on a short dataset ($T=375$) and 1000 models are trained on a long                                                                                        dataset ($T=7500$). Both are then tested on the same test data ($T=2500$). Model runs where excluded if the 1-step PE $>$ 1 on the training data.}
\label{tab:main_run_results}
\begin{tabular}{lll}
\toprule
metric & Short Training data & Long Training data \\
\midrule
$D_{stsp}$ & $3.83 \pm 6.42$ & $3.23 \pm 14.81$ \\
$D_{PSE}$ & $0.30 \pm 0.11$ & $0.32 \pm 0.13$ \\
1-step PE & $0.10 \pm 0.02$ & $0.06 \pm 0.01$ \\
5-step PE & $1.14 \pm 0.31$ & $0.76 \pm 0.09$ \\
10-step PE & $1.63 \pm 0.36$ & $1.53 \pm 0.22$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/HyperparameterSettings.tex <==
\end{table}
\begin{table}[ht]
\centering
\begin{{tabular}}{{|c|c|}}
\hline
Hyperparameter & Value \\ \hline
latent_dim & 16 \\
gaussian_noise_level & 0.05 \\
path_to_artifacts &  \\
optimizer & RADAM \\
batch_size & 16 \\
start_lr & 0.001 \\
batches_per_epoch & 50 \\
model & clippedShallowPLRNN \\
hidden_layers &  \\
D_stsp_bins & 30 \\
observation_model & Identity \\
lat_model_regularization & 0.0 \\
end_lr & 1e-06 \\
device & cpu \\
gradient_clipping_norm & 10.0 \\
num_bases & 0 \\
TR & 0.5 \\
hidden_dim & 50 \\
cut_r & 0.5 \\
sequence_length & 200 \\
MAR_ratio & 0.0 \\
obs_model_regularization & 0.0 \\
epochs & 1000 \\
MAR_lambda & 0.0 \\
cut_l & 0.25 \\
weak_tf_alpha & 0.2 \\
min_conv_noise & 5e-06 \\
train_test_split & 0.75 \\
\hline
\end{tabular}
\end{table}

==> tables/complete_main_run_results.tex <==
\begin{table*}[!ht]
\centering
\caption{Results of the PLRNN with BOLD observation model on the LEMON dataset. Model runs where excluded if the 1-step PE $>$ 1 on the training data.}
\label{tab:main_run_results}
\begin{tabular}{lllllll}
\toprule
 &  & $D_{stsp}$ & $D_{PSE}$ & 1-step PE & 5-step PE & 10-step PE \\
\midrule
\multirow[c]{2}{*}{$\ell=512$} & Train Data & $8.02 \pm 9.15$ & $0.44 \pm 0.16$ & $0.17 \pm 0.21$ & $0.42 \pm 0.32$ & $0.78 \pm 0.50$ \\
 & Test Data & $6.16 \pm 9.34$ & $0.25 \pm 0.11$ & $0.42 \pm 3.28$ & $1.35 \pm 5.54$ & $1.79 \pm 0.85$ \\
\midrule
\multirow[c]{2}{*}{$\ell=50$} & Train Data & $1.19 \pm 1.31$ & $0.21 \pm 0.05$ & $0.06 \pm 0.07$ & $0.30 \pm 0.26$ & $0.41 \pm 0.33$ \\
 & Test Data & $2.74 \pm 1.10$ & $0.14 \pm 0.03$ & $0.17 \pm 0.33$ & $1.20 \pm 0.41$ & $1.78 \pm 0.38$ \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/corr_diff_set_aln.tex <==
\iffalse
\begin{table}[ht!]
\centering
\caption{Pearson correlation coefficients between DSR measures evaluated on different test sets.}
\vskip 0.15in
\label{tab:corr_diff_set_ALN}
%\begin{NiceTabular}{l|l|l|lllll}
\begin{tabular}{l|l||lllll}
%
%& \multicolumn{2}{l}{observation}& \multicolumn{2}{l}{latent}\\
%metric & total  & test & total &test \\
\toprule
\multicolumn{2}{l}{Setting}& $D_{stsp}$ & $D_{PSE}$ & $PE_1$ & $PE_5$ & $PE_{10}$\\
\midrule
%\multirow{2}*{obs. / latent} &Short test & 0.96 & 0.47 & 0.47 & 0.68 & 0.69\\
\multirow{2}*{obs. / latent} & empirical test set & 0.96 & 0.47 & 0.47 & 0.68 & 0.69\\
%&Full experimental & $0.99$ & $0.88$ & 0.66 & 0.78 & $0.83$\\
&Full empirical & $0.99$ & $0.88$ & 0.66 & 0.78 & $0.83$\\
\midrule
%\multirow{2}*{short / long} & test& 0.84 & 0.37 & 0.71& 0.77 & 0.67\\
\multirow{2}*{empirical test set / GT test set} & test& 0.84 & 0.37 & 0.71& 0.77 & 0.67\\
& total & 0.75 & 0.70 & 0.65 & 0.79 & 0.73\\
\midrule
%\multicolumn{2}{l}{test / total} & 0.8 & 0.54 & 0.47 & 0.64 & 0.52 \\
\multicolumn{2}{l}{empirical test / empirical full} & 0.8 & 0.54 & 0.47 & 0.64 & 0.52 \\

\bottomrule
\end{tabular}
\end{table}
\fi

\begin{table}[ht!]
\centering
\caption{Pearson correlation coefficients between DSR measures evaluated on different test sets (outliers were discarded using the IQR method).}
\vskip 0.15in
\label{tab:corr_diff_set_ALN}
%\begin{NiceTabular}{l|l|l|lllll}
\begin{tabular}{l|l||lllll}
%
%& \multicolumn{2}{l}{observation}& \multicolumn{2}{l}{latent}\\
%metric & total  & test & total &test \\
\toprule
\multicolumn{2}{l}{Setting}& $D_{stsp}$ & $D_{PSE}$  & $PE_{10}$\\
\midrule
\multirow{2}*{obs. / latent} & empirical test set & 0.96 & 0.47 & 0.69\\
&full empirical & $0.99$ & $0.88$ & $0.88$\\
\midrule
\multirow{2}*{short / long} & empirical test set& 0.84 & 0.37 &  0.67\\
& Full empirical& 0.81 & 0.72 &  0.8\\
\midrule
\multicolumn{2}{l}{empirical test set / full empirical} & 0.8 & 0.54 & 0.83 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/large_aln_results.tex <==
\begin{table}
\centering
\caption{Results of the small PLRNN with BOLD observation model on the aln dataset. Model runs where excluded if the 1-step PE $>$ 1. $N_{converged}=99$}
\label{tab:main_run_results}
\begin{tabular}{lll}
\toprule
metric & Train Data & Test Data \\
\midrule
$D_{stsp}$ & $0.40 \pm 0.55$ & $0.31 \pm 0.38$ \\
$D_{PSE}$ & $0.38 \pm 0.16$ & $0.36 \pm 0.13$ \\
1-step PE & $0.02 \pm 0.01$ & $0.02 \pm 0.01$ \\
5-step PE & $0.15 \pm 0.00$ & $0.20 \pm 0.01$ \\
10-step PE & $0.20 \pm 0.01$ & $0.24 \pm 0.01$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/large_main_run_results.tex <==
\begin{table}
\centering
\caption{Results of the large PLRNN with BOLD observation model on the LEMON dataset. Model runs where excluded if the 1-step PE $>$ 1. $N_{converged}=629$}
\label{tab:main_run_results}
\begin{tabular}{lll}
\toprule
metric & Train Data & Test Data \\
\midrule
$D_{stsp}$ & $8.02 \pm 9.15$ & $6.16 \pm 9.34$ \\
$D_{PSE}$ & $0.44 \pm 0.16$ & $0.25 \pm 0.11$ \\
1-step PE & $0.17 \pm 0.21$ & $0.42 \pm 3.28$ \\
5-step PE & $0.42 \pm 0.32$ & $1.35 \pm 5.54$ \\
10-step PE & $0.78 \pm 0.50$ & $1.79 \pm 0.85$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/lemon_feature_cor_test.tex <==
\begin{table*}
\centering
\caption{Comparison of the correlations between the dynamical features of PLRNNs trained on the LEMON dataset.                                                             The unfiltered mean of all converged models is compared to the mean of models filtered for the lowest loss                                                             and for the lowest $D_{stsp}$. Models were excluded from the analysis if the 1-step PE $>$ 1.}
\label{tab:main_run_results}
\begin{tabular}{llllllll}
\toprule
& Feature & unfiltered mean r & filtered mean r & df & pvalue & significance \\
\midrule
\multirow[c]{7}{*}{Loss} & maximum LE $ \lambda_{max} $ & 0.121 & 0.084 & 10.043 & 0.512 &   \\
 & Kaplan-Yorke dimension & 0.112 & 0.138 & 9.722 & 0.659 &   \\
 & average velocity & 0.157 & 0.058 & 10.341 & 0.050 & * \\
 & Spectral norm $ W_1 $ & 0.190 & 0.285 & 11.369 & 0.016 & * \\
 & Spectral norm $ W_2 $ & 0.100 & 0.126 & 10.428 & 0.586 &   \\
 & Sum of diag($A$) & 0.034 & 0.034 & 13.044 & 0.974 &   \\
 & Sum of $h_1$ & 0.007 & 0.033 & 10.832 & 0.536 &   \\
\midrule
\multirow[c]{7}{*}{$D_{stsp}$} & maximum LE $ \lambda_{max} $ & 0.121 & 0.288 & 11.483 & $<$0.001 & *** \\
 & Kaplan-Yorke dimension & 0.112 & 0.257 & 10.741 & 0.005 & ** \\
 & average velocity & 0.157 & 0.241 & 10.572 & 0.063 & (*) \\
 & Spectral norm $ W_1 $ & 0.190 & 0.295 & 11.126 & 0.011 & * \\
 & Spectral norm $ W_2 $ & 0.100 & 0.096 & 10.690 & 0.912 &   \\
 & Sum of diag($A$) & 0.034 & 0.077 & 10.780 & 0.313 &   \\
 & Sum of $h_1$ & 0.007 & 0.092 & 10.412 & 0.093 & (*) \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/lin_conv_lemon_comparison.tex <==
\begin{table}
\centering
\caption{Comparison of convDSR and linDSR on the LEMON dataset. Model runs were excluded if the 1-step PE $>$ 1.}
\label{tab:main_run_results}
\begin{tabular}{lll}
\toprule
metric & ConvDSR & Linear \\
\midrule
$D_{stsp}$ & $2.74 \pm 1.10$ & $2.76 \pm 4.51$ \\
$D_{PSE}$ & $0.14 \pm 0.03$ & $0.15 \pm 0.03$ \\
1-step PE & $0.17 \pm 0.33$ & $0.12 \pm 0.04$ \\
5-step PE & $1.20 \pm 0.41$ & $1.15 \pm 0.26$ \\
10-step PE & $1.78 \pm 0.38$ & $2.00 \pm 0.44$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/short_long_aln_comparison.tex <==
\begin{table}
\centering
\caption{Results of the convDSR model on the ALN dataset. 1,000 models are trained on a short dataset ($T=375$) and a long dataset ($T=7,500$). Both are then tested on the same test data ($T=2,500$). Model runs where excluded if the 1-step PE $>$ 1 on the training data.}
\label{tab:main_run_results}
\begin{tabular}{lll}
\toprule
metric & Short training data & long training data \\
\midrule
$D_{stsp}$ & $3.83 \pm 6.42$ & $3.23 \pm 14.81$ \\
$D_{PSE}$ & $0.30 \pm 0.11$ & $0.32 \pm 0.13$ \\
1-step PE & $0.10 \pm 0.02$ & $0.06 \pm 0.01$ \\
5-step PE & $1.14 \pm 0.31$ & $0.76 \pm 0.09$ \\
10-step PE & $1.63 \pm 0.36$ & $1.53 \pm 0.22$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/small_aln_results.tex <==
\begin{table}
\centering
\caption{Results of the small PLRNN with BOLD observation model on the aln dataset. Model runs where excluded if the 1-step PE $>$ 1. $N_{converged}=99$}
\label{tab:main_run_results}
\begin{tabular}{lll}
\toprule
metric & Train Data & Test Data \\
\midrule
$D_{stsp}$ & $0.40 \pm 0.55$ & $0.31 \pm 0.38$ \\
$D_{PSE}$ & $0.38 \pm 0.16$ & $0.36 \pm 0.13$ \\
1-step PE & $0.02 \pm 0.01$ & $0.02 \pm 0.01$ \\
5-step PE & $0.15 \pm 0.00$ & $0.20 \pm 0.01$ \\
10-step PE & $0.20 \pm 0.01$ & $0.24 \pm 0.01$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/small_large_lemon_comparison.tex <==
\begin{table}
\centering
\caption{Comparison of PLRNNs with different hidden dim $\ell$ on the LEMON dataset. Model runs where excluded if the 1-step PE $>$ 1.}
\label{tab:main_run_results}
\begin{tabular}{lll}
\toprule
metric & $\ell=50$ & $\ell=512$ \\
\midrule
$D_{stsp}$ & $2.74 \pm 1.10$ & $6.16 \pm 9.34$ \\
$D_{PSE}$ & $0.14 \pm 0.03$ & $0.25 \pm 0.11$ \\
1-step PE & $0.17 \pm 0.33$ & $0.42 \pm 3.28$ \\
5-step PE & $1.20 \pm 0.41$ & $1.35 \pm 5.54$ \\
10-step PE & $1.78 \pm 0.38$ & $1.79 \pm 0.85$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/small_main_run_results.tex <==
\begin{table}
\centering
\caption{Results of the small PLRNN with BOLD observation model on the LEMON dataset. Model runs where excluded if the 1-step PE $>$ 1. $N_{converged}=1007$}
\label{tab:main_run_results}
\begin{tabular}{lll}
\toprule
metric & Train Data & Test Data \\
\midrule
$D_{stsp}$ & $1.19 \pm 1.31$ & $2.74 \pm 1.10$ \\
$D_{PSE}$ & $0.21 \pm 0.05$ & $0.14 \pm 0.03$ \\
1-step PE & $0.06 \pm 0.07$ & $0.17 \pm 0.33$ \\
5-step PE & $0.30 \pm 0.26$ & $1.20 \pm 0.41$ \\
10-step PE & $0.41 \pm 0.33$ & $1.78 \pm 0.38$ \\
\bottomrule
\end{tabular}
\end{table}

